Towards Scalable Network Delay Minimization

Reduction of end-to-end network delays is an optimization task with applications in multiple domains. Low delays enable improved information flow in social networks, quick spread of ideas in collaboration networks, low travel times for vehicles on road networks and increased rate of packets in the case of communication networks. Delay reduction can be achieved by both improving the propagation capabilities of individual nodes and adding additional edges in the network. One of the main challenges in such design problems is that the effects of local changes are not independent, and as a consequence, there is a combinatorial search-space of possible improvements. Thus, minimizing the cumulative propagation delay requires novel scalable and data-driven approaches. In this paper, we consider the problem of network delay minimization via node upgrades. Although the problem is NP-hard, we show that probabilistic approximation for a restricted version can be obtained. We design scalable and high-quality techniques for the general setting based on sampling and targeted to different models of delay distribution. Our methods scale almost linearly with the graph size and consistently outperform competitors in quality.

==> 5.1_expold.tex <==
%-----------------%%%%%%%%%%%%%% SMALL GRAPH FIGURES-----------------------

\begin{figure*}[t]
    \centering
 %  \subfloat[Synth-2K]{\includegraphics[width=0.25\textwidth]{figures/Experiments/uniform/PCS_effi_2000.eps}\label{fig:PCS_effi_2000}}
  %  \subfloat[Synth-2K]{\includegraphics[width=0.25\textwidth]{figures/Experiments/uniform/PCS_qual_2000.eps}\label{fig:PCS_qual_2000}}
    \subfloat[Traffic-Uniform]{\includegraphics[width=0.25\textwidth]{figures/Experiments/uniform/PCS_effi_traffic.eps}\label{fig:PCS_effi_traffic}}
    \subfloat[Traffic-Uniform]{\includegraphics[width=0.25\textwidth]{figures/Experiments/uniform/PCS_qual_traffic.eps}\label{fig:PCS_qual_traffic}}
    \subfloat[Traffic-Delay]{\includegraphics[width=0.25\textwidth]{figures/Experiments/general/GS_effi_traffic.eps}\label{fig:GS_effi_traffic}}
    \subfloat[Traffic-Delay]{\includegraphics[width=0.25\textwidth]{figures/Experiments/general/GS_qual_traffic_sp74.eps}\label{fig:GS_qual_traffic_sp74}}
  %  \subfloat[Traffic-Delay B]{\includegraphics[width=0.25\textwidth]{figures/Experiments/general/GS_qual_traffic_sp87.eps}\label{fig:GS_qual_traffic_sp87}}
 %   \subfloat[Traffic-Delay C ]{\includegraphics[width=0.25\textwidth]{figures/Experiments/general/GS_qual_traffic_sp100.eps}\label{fig:GS_qual_traffic_sp100}}
    \caption{\small Comparison of baselines and (a-b) PCS in the \textit{Uniform Model}; and (c-d) GS in the \textit{General Model} on Traffic. \label{fig:baselines_small_large}}
\vsc \end{figure*}

%\subsection{Performance of Our Sampling Schemes}
%In this section we evaluate the quality of our proposed methods. 
\subsection{Quality of sampling compared to Greedy}
We report the number of samples in PCS and GS as $c*logn$, where $c$ is related to the expected error $\epsilon$ in Thms.~\ref{thm:approxgeneral} and \ref{thm:approxpathcount}. Unless stated otherwise, we use $c=10$. 

First, we compare our sampling schemes GS and PCS with Greedy (GR) in order to evaluate the effect of sampling on quality, which we theoretically analyze in Thms. \ref{thm:approxgeneral}, \ref{thm:approxpathcount}. To enable the comparison, we use small real datasets due to the limited scalability of GR. 
%We evaluate the accuracy and efficiency of our algorithms on small networks. 
%Networks used for evaluation include Traffic and a BA synthetic network with $2000$ vertices and rate of growth: $5$ edges per node. %In small networks, computing the sum of shortest paths between all pairs of vertices is easier. 
The quality of the compared algorithms is quantified as the Relative Reduction (RR) of SPD, while efficiency---in terms of wall-clock time. We use $3.5logn$ samples for GS and PCS in these experiments.

In all experiments, our sampling schemes achieve similar quality as that of Greedy (GR), while taking close to two orders of magnitude less time. In the uniform model, the difference in quality between our sampling scheme PCS and GR does not exceed $.05\%$ in traffic dataset (Fig.~\ref{fig:PCSGR_qual_traffic}), while PCS takes only $2\%$ of the time taken by GR (Fig.~\ref{fig:PCSGR_effi_traffic}). 
This trend persists in the case of the general delay model for which we employ our sampling-based Greedy (GS). 
%In synthetic networks with uniformly chosen random delay,
%the quality of GS is within $3\%$ of that of GR, while its running time is only $1.5\%$ of the time taken by GR (Fig. \ref{fig:GSGR_effi_2000_500-1000},\ref{fig:GSGR_qual_2000_500-1000}).
We compare GS and GR on multiple snapshots of the Traffic dataset and report average completion times and quality in Fig. \ref{fig:GSGR_effi_traffic_sp1},\ref{fig:GSGR_qual_traffic_sp1}. GS is $200$ times faster than GR and its solution's RR is only $0.1\%$ worse than that of GR Figs.~\ref{fig:GSGR_effi_traffic_sp1},\ref{fig:GSGR_qual_traffic_sp1}. We observe similar results in synthetic data (see the extended version \cite{medya2016}).

%\ref{fig:GSGR_effi_traffic_sp74},  \ref{fig:GSGR_qual_traffic_sp74}). 
%We also perform a synthetic network experiment with uniformly chosen random delays in the range $[500,1000]$.% ($DS1$) and (ii) in the range $[1500,2500]$. 
%\todo{unclear:} For this setting of vertex delays and network size (mentioned above), the number of paths through a vertex can be at most in the order of square of the network size. Other random settings of delay produce similar results (omitted due to space limitations).


\begin{table}[t]
\vspace{-1mm}
\centering
\scriptsize
\begin{tabular}{| c | c | c | c | c | c |}

\hline
&\multicolumn{3}{c|}{\textbf{Quality RR(\%)}} & \multicolumn{2}{c|}{\textbf{Time [sec.]}}\\
\hline

\textbf{Airlines}& GR& GS& High-Delay & GS & GR\\
\hline
\textbf{JB}& $68.3$ & $68.2$ &  $63.9$ & $0.1$ & $0.22$\\
\hline
\textbf{SA}&$58.5$ &  $58.3$ &  $58.5$ & $0.4$ & $0.53$\\
\hline
\textbf{AA}& $55$ & $54.3$ &  $5.45$ & $0.06$ & $0.9$\\
\hline
\textbf{DA}& $48.9$ & $48.4$ &  $4.44$ & $0.4$ & $0.8$\\
\hline
\end{tabular}
\vspace{-1mm}
\caption{ \small Comparison on the airlines dataset. For budget $5$, columns 2-4 show the RR for GR, GS, and High-Delay respectively and columns 5-6 show running times. \label{table:results_airlines}}
\vspace{-1mm}
 \end{table}


%\textbf{Airlines data:} 
In the airline data we assign node delay as the average airline-induced delay of all historical flights originating from an airport. Table~\ref{table:results_airlines} summarizes our results. GS matches the quality of GR in a fraction of computation time. For AA, our solution selects important nodes which are central and also have significant delays. The solution contains hub airports like those in Dallas, Charlotte and Phoenix, since improving these airports make them more central in the network and collectively improve the total end-to-end delay by $55\%$~\ref{fig:AA}. Surprisingly, considering only node delay (baseline "High-Delay") has significant disadvantages. Some non-central airports in the AA and DA networks have significant average delays and hence disregarding the network position of upgrade candidate results in a $10$-fold worse quality of the High-Delay baseline. All other baselines do not exceed the quality of GS for varying budgets and airlines (comparisons omitted due to space constraints).%  are distributed within a very low range and central nodes have the high delays. %Though it is a local property of nodes, High-Delay produces exact same solution as GR.


\begin{table}[t]
\centering
\scriptsize
\begin{tabular}{| p{1.2cm} | p{1.5cm} |p{1.8cm}| p{2.3cm} |}
\hline
\textbf{Algs.}& \textbf{Selection} & \textbf{Uniform} & \textbf{General}\\
\hline
Random & $10$ trials  & O(n) & O(n) \\\hline
Deg-Cen & Degree & O(nlogn) & O(nlogn) \\ \hline
High-Delay & Delay & O(nlogn)) &O(nlogn) \\\hline
Path-Cen\cite{dilkina2011} & Delay$\times$\#SPs & O(n(m+n)) & O(n(m+nlogn))\\\hline
It-Path-Cen\cite{dilkina2011} &  Delay$\times$\#SPs w. updates  & O(kn(m+n)) & O(kn(m+nlogn)) \\\hline
PCS & Alg.~\ref{algo:PCS} & O(kc(m+n)logn) & \\\hline
GS & Alg.~\ref{algo:GS}  &  & O(kc(m+nlogn)logn) \\\hline
GR & Alg.~\ref{algo:GR}  & O(k$n^3$) & O(k$n^3$) \\\hline
\end{tabular}
\vspace{-1mm}
\caption{\small Theoretical complexity of compared algorithms.}\label{tab:baselines}
%\vspace{-1mm}
\vsc \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LARGE GRAPH FIGURES

\begin{figure*}[t]
    \centering
%\subfloat[Quality vs $\#$Sample]{\includegraphics[width=0.25\textwidth]{figures/Experiments/large/twitter_celeb-qual_sample.eps}\label{fig:twitter_celeb_qual_sample}}
%\subfloat[Time vs $\#$Sample]{\includegraphics[width=0.25\textwidth]{figures/Experiments/large/twitter_celeb_time_sample.eps}\label{fig:twitter_celeb_time_sample}}
\subfloat[Twitter-Celeb]{\includegraphics[width=0.2\textwidth]{figures/Experiments/large/twitter_celeb_qual.eps}\label{fig:twitter_celeb_qual}}
\subfloat[Twitter-Politics]{\includegraphics[width=0.2\textwidth]{figures/Experiments/large/twitter_politics_qual.eps}\label{fig:twitter_politics_qual}}
\subfloat[Twitter-Science]{\includegraphics[width=0.2\textwidth]{figures/Experiments/large/twitter_sci_qual.eps}\label{fig:twitter_science_qual}}
\subfloat[DBLP-Random]{\includegraphics[width=0.2\textwidth]{figures/Experiments/large/dblp_qual.eps}\label{fig:dblp_random_qual}}
\subfloat[Uniform]{\includegraphics[width=0.2\textwidth]{figures/Experiments/large/PCS_budget5.eps}\label{fig:PCS_budget5}}
\vspace{-2mm}
   \caption{ \small (a-d) General Model:  Quality of GS and baselines on Twitter-Celeb, Twitter-Politics, Twitter-Science and DBLP. (e) Uniform Model: Quality of PCS and baselines for budget=5 on DBLP, Twitter-Politics and Twitter-Celeb.\label{fig:large}}
\vsc \end{figure*}

%----------------------------------------------------------------------------------

\vspace{-2mm}
\subsection{Comparison to baselines}\label{sec:baselines}
Next we evaluate the performance of our algorithms in comparison to alternatives. We consider several baseline methods, listed in Tab.~\ref{tab:baselines} along with their theoretical running times and those of our algorithms. Some baselines select TS vertices based on local properties: degree (Deg-Cen) or delay (High-Delay); while others---based on the product of global path centrality and delay (Path-Cen and It-Path-Cen~\cite{dilkina2011}). It-Path-Cen updates the number of shortest paths through a vertex after each selection of a target vertex. 
 % The main advantage of using small networks is the lower computation time of sum of the shortest paths between every pair of vertices. Thus we are able to test our algorithms based on exact metric to optimize.
%\noindent \textbf{Comparisons on small graphs:} \todo{there are too many figures showing GS and PCS only marginally better. We should focus more on settings where we do much better.}
%Figures \ref{fig:PCS_qual_2000} and \ref{fig:PCS_qual_traffic} show the computation times and relative reduction for the uniform model in synthetic graphs. We use $50log(n)$ samples for PCS in this case. Note that, the baseline algorithm It-Path-Cen is equivalent to GR for the uniform model (comparison results already available in Fig.~\ref{fig:GSGR_comparison}). %For the synthetic dataset, Deg-Cen produces similar results (within $0.1\%$) as PCS (Fig.~\ref{fig:PCS_qual_2000}), because when the delays are uniform, one can expect that shortest paths often pass through vertices with high degree. 
%\todo{this is kind of a weak statement} In Traffic PCS produces at least $6\%$ better RR than Deg-Cen does. 

%GS uses $10log(n)$ in Traffic with three different snapshots of speeds (Fig.~\ref{fig:GS_qual_traffic_sp74}, \ref{fig:GS_qual_traffic_sp87}, \ref{fig:GS_qual_traffic_sp100}). It produces higher RR than both Path-Cen and It-Path-Cen, with 10- and 100-times running time improvement respectively. 
%As Path-Cen does not recompute the shortest paths after each selection, its quality deteriorates for increasing budget. 
%Unlike It-path-Cen, our approach GS does not assume probable target nodes being on shortset paths and hence it has better quality. In all three different snapshots of Traffic, the efficiency of the algorithms are similar (average efficiency is presented in Fig.\ref{fig:GS_effi_traffic}).

Figures~\ref{fig:PCS_effi_traffic},~\ref{fig:PCS_qual_traffic} present the experimental running times and relative delay reduction (RR) of competing techniques on the Traffic network with uniform delays using $50log(n)$ samples for PCS. The baseline algorithm It-Path-Cen for the setting of uniform delays is equivalent to the exhaustive greedy GR and this comparison is already available in Fig.~\ref{fig:GSGR_comparison}. On this relatively small network, PCS produces at least $6\%$ better RR than the best alternative Path-Cen, while taking a similar time to evaluate. Note, that in this setting simple alternatives such as Random and Deg-Cen, although fast, have unacceptably low quality.

Next we associate the delays at road intersections, measured at different times, with network nodes and compare the performance of competing techniques. In this general delay model, our GS sampling technique uses $10log(n)$ samples. As the results on different snapshots are similar, we present representative figures on efficiency and quality (Fig.~\ref{fig:GS_effi_traffic}, \ref{fig:GS_qual_traffic_sp74}). GS produces higher RR than both Path-Cen and It-Path-Cen, with up to 1 and 2 orders of magnitude running time improvement respectively. 
%As Path-Cen does not recompute the shortest paths after each selection, its quality deteriorates for increasing budget. 
Unlike It-path-Cen, GS does not target nodes simply based on the number of shortest paths through them, but estimates the improvement of nodes given those already in the target set and achieves a better quality for significantly shorter running time.

In larger graphs computing the exact quality (reduction of SPD) has high computational cost as it requires computing all-pair shortest paths. Hence, in order to evaluate the competing techniques, we estimate RR based on a representative sample of pairwise shortest path lengths as opposed to all pairs. We randomly sample $1000$ pairs $10$ times and average the quality results. We evaluate the competing techniques on DBLP and the Twitter datasets.
%\todo{if time allows we should show the standard deviation with error bars}

First we evaluate the running time in comparison to the best-quality competing techniques in Tab.~\ref{tab:scale_dilkina}. As expected based on their theoretical complexity, Path-Cen and It-Path-Cen~\cite{dilkina2011} do not scale well for large datasets. Our algorithms complete in at most $36$ min, while the alternatives take close to or more than $5$h on the same input (DNF stands for ``does not finish in $5$ hours''). Twitter-50K in this experiment is a subgraph of the Twitter-Politics network involving 50K nodes, while in the uniform-delay setting we evaluate PCS on a subgraph of DBLP of 100K nodes (DBLP-100K). 

Since the methods by Dilkina et al.~\cite{dilkina2011} do not scale for large graphs we compare the quality of our sampling schemes with that of Deg-Cen and High-Delay on the full large-graph datasets (High-Delay is replaced by Random in the uniform model experiments as delays in this setting are equal). To enable even higher scalability for GS, we use multi-threading with $4$ threads to compute the shortest paths (steps $4-7$ in Alg.~\ref{algo:GS}). %We denote this multi-threaded version of GS as \textit{GS(4T)}. 
For the rest of the experiments, we use GS(4T).


%%%%%%%%%%%%%%%%%%TABLES-------------------
\begin{table} [t]
\centering
\scriptsize
\begin{tabular}{| c | c | c | c |c |}
\hline
\textbf{Data}& PCS& GS & Path-Cen & It-Path-Cen\\
\hline
%\textbf{DBLP-100K (general)}&$0.6$& $.09$  & DNF & DNF\\
%\hline
%\textbf{Twitter-50K (uniform)}& $.03$ &- &$4.5$ & DNF\\
DBLP-100K (unif.)&$2$ m& $-$ & $4.5$ h & DNF\\
\hline
Twitter-50K (gen.)&$-$  &$36$ m& DNF & DNF\\
\hline
\end{tabular}
\vspace{-1mm}
\caption{\small Running time comparison of our algorithms and those proposed in~\cite{dilkina2011} (budget = $5$).}\label{tab:scale_dilkina}
 \end{table}


\begin{table} [t]
\vspace{-1mm}
\centering
\scriptsize
\begin{tabular}{| c | c | c | c |}
\hline
\textbf{Data}& Algo. & $\#$Sample & Time(min)\\
\hline
Twitter-Celeb (unif.)& PCS & $148$ & $2.5$\\
\hline
Twitter-Politics (unif.)& PCS & $166$ & $3.5$\\
\hline
DBLP (unif.)& PCS & $200$ & $9$\\
\hline
Twitter-Celeb (gen.)& GS(4T) & $148$ & $1$\\
\hline
Twitter-Politics (gen.)& GS(4T) & $64$ & $19$\\
\hline
Twitter-Science (gen.)& GS(4T) & $64$ & $12$\\
\hline
DBLP (gen.)& GS(4T) & $40$ & $62$\\
\hline
\end{tabular}
\vspace{-1mm}
\caption{\small Running times on DBLP and Twitter data, budget = $5$ of PCS and GS(4T).}\label{tab:time_GS(4T)_PCS}
\vspace{-2mm}
\vsc \end{table}

Tab.~\ref{tab:time_GS(4T)_PCS} presents the running times of our algorithms in both the uniform and general delay settings together with the number of sampled pairs of each run over the full networks. The number of samples $clog(n)$ depends on both the size of the network and the constant $c$ (which we set to values not exceeding $20$). In the uniform scenario (datasets denoted \textit{unif.}), we assume delay $1$ associated with nodes. PCS completes in the order of minutes in uniform-delay networks and GS within 62 minutes on the largest DBLP dataset.

Figs.~\ref{fig:twitter_celeb_qual}-\ref{fig:dblp_random_qual} show the quality of GS in Twitter and DBLP. In all cases GS performs better than alternatives for increasing budget, since the alternatives fail to capture the dependency between upgraded nodes and are limited to local node properties. We get higher quality in Twitter-Celeb as we use relatively higher number of samples. The RR in DBLP is relatively low due to the large network size and disproportionately small budgets ($5$ and $10$ out of $1.1M$ nodes). Fig.~\ref{fig:PCS_budget5} presents an analogous comparison for uniform delay. Our technique PCS outperforms alternative in Twitter (budget $k=5$). In DBLP, Deg-Cen has similar quality to that of PCS since authors of high degree tend to be central.

The only parameter in our techniques is the number of samples which provides a natural trade-off between running time and quality. Our analysis shows that we usually need only small fraction of sampled pairs to match the performance in greedy in both real-world and synthetic data. Details of this analysis in real world data are available in the extended version of the paper~\cite{medya2016}.

%In the case of DBLP, we perform experiments with delays from the Data Management (DM) field. We set the delay to $0$ for authors who have no or small ($<5$) number of papers in DM (we need enough observations to estimate the delay). As a result non-zero delays in the full network involving authors from all fields are very rare, limiting the possible reduction of delay overall. Furthermore, the random pairs selected to evaluate the reduction do not necessary capture the differences among alternatives (Note: all pairs evaluation for this network is infeasible). Hence, we use the full network for running-time evaluation and focus on quality in a $15K$-node subgraph obtained using BFS from a prolific ($>100$ papers) DM researcher. GS in this subgraph produces $17\%$ higher reduction than alternatives. 

%%TODO- add some of the names chosen by High-Degree and Ours






%%%










